Identity-Consistent Analysis of Long-Shot Windsurfing Video: A Domain-Specific Offline Tracking System

Long-shot windsurfing video combines small targets, large camera pans, prolonged overlaps, and rapidly changing backgrounds. The desired output is not a generic MOT trace but a separate, stable rider-relative video for each surfer; one false identity merge can invalidate an otherwise useful result. We present an offline analysis system that detects surfers, forms conservative local tracklets, links them globally with camera-compensated motion and a foreground-masked sail-color descriptor, and uses two pose keypoints on the rig to drive a rider-relative virtual camera. The tracking stage is evaluated on 21 manually reconstructed development videos containing 41,004 retained observations. On this fixed-observation protocol, the production system achieves 0.957 pairwise precision, 0.918 recall, and 0.937 F1, compared with 0.792 F1 for OC-SORT and 0.828 for BoT-SORT. Compared with OC-SORT, it reduces fragmentation excess from 845 to 42, but nine of its 95 output tracks mix rider identities and these errors affect seven of the 21 videos.

==> sections/player.tex <==
\section{Frame-Accurate Delivery}
\label{sec:player}

Identity-consistent tracks are useful only if the browser applies metadata to the
frame that produced it. Ordinary HTML video exposes media time rather than stable
frame identity, so the WebCodecs path~\cite{webcodecs} defines a canonical index by
ordering packets by presentation timestamp and sequence number. Preview seeks from a
preceding keyframe and decodes forward. Export decodes independently but maps each
sample to the same index, resynchronizing by timestamp when necessary. The shared
index and crop geometry preserve frame correspondence through preview and export;
this is a delivery constraint rather than a tracking contribution.

